A Novel Approach to Solve K-Center Problems with Geographical Placement

The facility location problem is a well-known challenge in logistics that is proven to be NP-hard. In this paper we specifically simulate the geographical placement of facilities to provide adequate service to customers. Determining reasonable center locations is an important challenge for a management since it directly effects future service costs. Generally, the objective is to place the central nodes such that all customers have convenient access to them. We analyze the problem and compare different placement strategies and evaluate the number of required centers. We use several existing approaches and propose a new heuristic for the problem. For our experiments we consider various scenarios and employ simulation to evaluate the performance of the optimization algorithms. Our new optimization approach shows a significant improvement. The presented results are generally applicable to many domains, e.g., the placement of military bases, the planning of content delivery networks, or the placement of warehouses.

==> content/requirements.tex <==
\section{REQUIREMENTS}\label{sec:requirements}
Starting from our use case, we know the geographical location of the to be supplied vertices and the precise infrastructure with edges between them.
%These information of a specific scenario need to be transformed to an abstract model. This is necessary for the optimization of the center node placement and for the simulation with different amount of center nodes.
Dependent on the scenario, the objective function, the metrics, and the placement constrains need to be specified.
%This again has a large influence on the used infrastructure, possible placement locations and the evaluation with the objective function.
%For the geographical placement the distance of a vertice to its nearest center node is of main importance. It is mandatory to define the objective criterion for the optimization of the placement. Typical objectives include: maximum, quantile 95\% and median as well as average values.
%Another possible and highly relevant objective for the management of a company is a function that tests whether all distances are smaller than a specified limit, to guarantee a certain quality.

%Beside these metrics for the optimization, it is important to know general aspects for a provider.
Before a concrete planning of the provided service can take place, the amount of corresponding center nodes and their locations must be analyzed to achieve a specified objective. % The placement of the warehouses needs planning against realistic conditions.
A corresponding flexible and powerful optimization algorithm is necessary for this. The algorithm does not need to be necessarily very fast. A good result is substantially more important, because the decision has a strong and long term influence on the future.

According to the scenario and various application areas, we address the geographical facility placement problem concerning to the following main aspects:
\begin{itemize}
%\item Decision on a meaningful evaluation measure. 
\item High performance and adaptable placement algorithm. % for realistic conditions %for the extension of an existing supply chain.
\item Meta-Optimization to identify the necessary amount of center for a specific scenario to reach a predefined quality.
\item Performance differences between the constraint free and the node placement. (Influence of decisions.)
\item Placement of central nodes in relation to the number of vertices to be supplied, the distribution area, and their distance.
\end{itemize}



% Diesen Absatz eventuell weglassen.
%As one of the first steps of an effective management planing process, it is necessary to analyze the existing transportation infrastructure and the location of the estimated customers. Several transportation paths differ in length, time consumption, and utilization as well as quality, robustness and maybe service charge like toll. These properties of a sub path have to be abstracted to different weights in our model. Also several customers can have weights to represent the relative importance of the company for example premium customers.


